Reward Biased Maximum Likelihood Estimation for Learning in Constrained MDPs

We use the Reward Biased Maximum Likelihood Estimation (RBMLE) algorithm to learn optimal policies for constrained Markov Decision Processes (CMDPs). We analyze the learning regrets of RBMLE.

==> subsecs/Garbage/compute_May18.tex <==
\section{Solving~\eqref{eq:rbmle_2} Efficiently}\label{sec:solve_cmdp}
We will see how to solve the following problem efficiently:
\begin{align}
	&\te_k \in \arg\max_{\te \in \Theta} \bigg\{ \max_{\pi \in \Pi_{S}}\bigg\{ \alpha(\tau_k) \bar{r}(\theta,\pi) -\sum_{(x,u)} n_k(x,u)KL\left( \hat{p}_{k}(x,u),\te(x,u)  \right): \bar{c}(\te,\pi) \le c_{ub} \bigg\} \bigg\},\label{rbmle_prob}
\end{align}
and also obtain the corresponding optimal $\pi$.

\textbf{Embedding into an extended CMDP}: 
The problem~\eqref{rbmle_prob} can be viewed as an extended CMDP in which the optimizer\slash controller has to choose the following two quantities at each time $t$: \\
(i) controls $u(t)$, \\
(ii) MDP parameters $\te $.\\
We can merge these two controls, and let $u^{+}(t):= (u(t),\te(t))\in U \times \Theta$ be the controls for this \textit{extended CMDP}. The controlled transition probabilities for this extended MDP are given as follows (note that $\te$ is also part of control):
\ali{
	P^{+}(x,u^{+},y) =  \te(x,u,y),\label{def:extend_ptm}
}
where 
\nal{
	u^+ = (u,\te).
}


Consider the following linear program in which the decision variables are given by $\{ \mu(x,u,\te): x \in \cX, u \in \cU,\te \in \widetilde{\Theta}_{\epsilon} \}$:
\begin{align}
	&\max \sum_{x \in \cX} \sum_{u \in \cU} \sum_{\te \in  \widetilde{\Theta}_{\epsilon}} \mu(x,u,\te)r(x,u),\label{overallobj_appx}
	&\intertext{subject to }\notag\\
	& \sum_{(u,\te)} \mu(x,u,\te) = \sum_{(y,v,\te)} \mu(y,v,\te) P^{+}(y, (v,\te),x), \label{const1n_appx} \\
	& \mu(x,u,\te) \geq 0, \\
	&\sum_{x \in \cX}\sum_{u} \sum_{\te \in  \widetilde{\Theta}_{\epsilon}}\mu(x,u,\te) = 1,  \label{const2n_appx} \\
	& \sum_{(x,u,\te)} \mu(x,u,\te) c(x,u) \leq U_B . \label{constall_appx}
\end{align} %\eqref{overallobj_appx}-\eqref{constall_appx}
Let $\mu\ust$ be an optimal solution. $\pi\ust$ be the policy that randomizes amongst $u\in \cU$ when state is $x$, as follows: 
\begin{align}
	\frac{  \sum\limits_{\te \in  \widetilde{\Theta}_{\epsilon}}    \mu\ust(x,u,\te)}{\sum_{(v,\te)} \mu\ust(x,v,\te)}.
\end{align}
(In case the denominator above is zero, choose any $\pi\ust_n(x_n,u_n,\te_n) \geq 0$ satisfying
$\sum_{v_n,\te_n} \pi\ust_n(x_n,v_n,\te_n) = 1$). 



\begin{definition}
	Let $\Pi^{+}_{S}$ denote the class of ``stationary randomized policies'' for the extended CMDP~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}. These policies fix $\te(t)\equiv \te,\forall t$ and also let $u(t)$ be solely a (possibly randomized) function of $x(t)$.
\end{definition}

\begin{lemma}\label{lemma:stat_opt}
	For the problem~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}, there exists an optimal controller within the class $\Pi^{+}_S$. 
\end{lemma}

\begin{comment}
We will approximate the infinite horizon CMDP~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2} by a finite time horizon problem that requires the agents to make decisions for $H$ steps. For this, we need the following assumption.

\begin{assumption}[Ergodicity]
The quantities 
\nal{
&\sup_{\pi^{+} \in \Pi^{+}_S} \Bigg| \bar{C}(\pi^{+})-\frac{1}{H}\bE_{\pi^{+}} \sum_{t=1}^{H}c(x(t),u(t))\Bigg|,\\
& \sup_{\pi^{+} \in \Pi^{+}_S} \Bigg|\bar{D}(\pi^{+})-\frac{1}{H}\bE_{\pi^{+}} \sum_{t=1}^{H}d(u(t))\Bigg|
}
are $o(H)$, i.e. their normalized (by $H$) versions vanish as $H\to\infty$. $\blacksquare$
\end{assumption}
%Let $\pi^{+,\star}$ be an optimal policy for the extended CMDP~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}. 

Under this assumption,~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2} can be approximated by the following problem involving $H$ horizon:
\ali{
\min_{\pi^+} \bE_{\pi^+}\left( \sum_{t=1}^{H} c(x(t),u^+(t))\right),\label{finite:obj}\\
\mbox{s.t.}\quad  \bE_{\pi^+}\left( \sum_{t=1}^{H} d(u^+(t)) \right)\le H U_B.  \label{finite:con}
}
Having reformulated~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}, we now derive some important structural results for it. 
\end{comment}
In~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}, the choice for $\te_n$ belongs to the set $\Theta_n$. Since~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2} has an uncountable action set, we will approximate it by a problem that involves finitely many decision variables. 




\textbf{Approximating Extended CMDP}: In what follows, we will assume that we have approximated the set $\Theta_n$ by a finite set $\tilde{\Theta}_n(\epsilon_1)$ that satisfies the following: for each $\te_n\in \Theta_n$ there exists at least one point $\tilde{\te}_n$ in the set $\tilde{\Theta}_n(\epsilon_1)$ that satisfies $\|\te_n-\tilde{\te}_n\|\le \epsilon_1$. 
We let $\tilde{\Pi}$ denote the set of policies that restrict to the set $\tilde{\Theta}_n(\epsilon_1)$ while choosing $\te_n$ (intead of choosing from a larger set $\Theta_n$). A policy $\tilde{\pi}\in \tilde{\Pi}$ chooses $u_n(t)\in \cU_n$ and $\te_n\in \tilde{\Theta}_n(\epsilon_1)$ for each agent $n$. The following assumption is in affect throughout this section.

\begin{assumption}\label{assum:strict}
	There exists a policy $\pi_{feas.} \in \tilde{\Pi}$ and a constant $\epsilon>0$ such that the average control cost under $\pi_{feas.}$ is strictly below $U_B - \epsilon$, where $U_B$ is as in the constraint~\eqref{def:constraints_learn_1}. We denote
	\ali{
		\eta := U_B - \epsilon - \bar{D}(\pi_{feas.}) \label{def:eta}
	}
\end{assumption}

The following CMDP that restricts to the class $\tilde{\Pi}$ is supposed to approximate the problem~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}:
\ali{
	\min_{ \tilde{\pi} \in \tilde{\Pi}} & \limsup_{T\to \infty} \frac{1}{T} \sum_{t=1}^{T} \bE_{\tilde{\pi}} \left( c(x(t),u(t)) \right)\label{cmdp_approx_obj}\\
	\mbox{ s.t. }& \limsup_{T\to \infty} \frac{1}{T} \sum_{t=1}^{T} \bE_{\tilde{\pi}} \left( d(x(t),u(t)) \right)  \le U_B.\label{cmdp_approx_con}
} %\eqref{cmdp_approx_obj}-\eqref{cmdp_approx_con}
\begin{theorem}\label{finite_LP}
	Consider the following linear program in which the decision variables are given by $\{ \mu_n(x_n,u_n,\te_n): x_n \in \cX_n, u_n \in\cU_n,\te_n \in \tilde{\Theta}_n(\epsilon_1), 1 \leq n \leq N \}$:
	\begin{align}
		&\min\sum_{n\in [N]} \sum_{x_n \in \cX_n} \sum_{u_n \in \cU_n} \sum_{\te_n \in \tilde{\Theta}_n(\epsilon_1)} \mu_n(x_n,u_n,\te_n) c_n(x_n,u_n) \label{overallobj_appx}
		&\intertext{subject to }\notag\\
		& \sum_{(u_n,\te_n)} \mu_n(x_n,u_n,\te_n) = \sum_{(y_n,v_n,\te_n)} \mu_n(y_n,(v_n,\te_n)  ) P^{+}_n(y_n, (v_n,\te_n)   ,x_n), \label{const1n_appx} \\
		& \mu_n(x_n,u_n,\te_n) \geq 0, \\
		&\sum_{x_n \in \cX_n}\sum_{u_n \in \cU_n} \sum_{\te_n \in \tilde{\Theta}_n(\epsilon_1) }\mu_n(x_n,u_n,\te_n) = 1, \forall n,  \label{const2n_appx} \\
		&\sum_{n\in [N]} \sum_{(x_n,u_n,\te_n)} \mu_n(x_n,u_n,\te_n) d_n(x_n,u_n) \leq U_B . \label{constall_appx}
	\end{align} %\eqref{overallobj_appx}-\eqref{constall_appx}
	Let $\mu\ust_n, ~n\in [N]$ be an optimal solution. Define the policy $\pi\ust_n$ as follows: 
	\begin{align}
		&\pi\ust_n(x_n,u_n) := \frac{\sum\limits_{\te_n \in \tilde{\Theta}_n}\mu\ust_n(x_n,u_n,\te_n)}{\sum_{(v_n,\te_n)} \mu\ust_n(x_n,v_n,\te_n)}.
	\end{align}
	(In case the denominator above is zero, choose any $\pi\ust_n(x_n,u_n,\te_n) \geq 0$ satisfying
	$\sum_{v_n,\te_n} \pi\ust_n(x_n,v_n,\te_n) = 1$). The policy $\otimes \pi^{\star}_n$ is optimal for the CMDP~\eqref{cmdp_approx_obj}-\eqref{cmdp_approx_con}.
\end{theorem}



The next result follows from Theorem~\ref{th:cho_meyer}.

\begin{lemma}
	Consider the finite LP~\eqref{overallobj_appx}-\eqref{constall_appx} that solves the CMDP~\eqref{cmdp_approx_obj}-\eqref{cmdp_approx_con}. The average reward satisfies 
	\nal{
		\tilde{r}(0) \ge     r\ust - \kappa_{\pi\ust} \epsilon - \kappa_{\pi\ust}\epsilon\frac{\hat{\eta}}{\eta} .
	}
\end{lemma}
\begin{proof}
	Let $\pi\ust$ solve the CMDP~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}. Under $\pi\ust$, in each state $x$, there is a probability measure over the space $\cU\times \Theta$ that corresponds to randomized choice of controls for the entire system, and the choice of the MDP parameter. We modify $\pi\ust$ as follows, so that now it chooses $\te_n$ from the finite set $\tilde{\Theta}_n$: when $\pi\ust$ suggests $\te_n$, then this is mapped to the nearest point $\tilde{\te}_n$ in the set $\tilde{\Theta}_n$. Clearly, we have that $\|\te_n-\tilde{\te}_n\|\le \epsilon$, and hence from Theorem~\ref{th:cho_meyer} that the average reward of this modified policy (say $\pi_{mod.}$) is greater than $r\ust -  \kappa_{\pi\ust} \epsilon $, and average cost is lesser than $U_B + \kappa_{\pi\ust} \epsilon$.
	\ali{
		\bar{r}(\pi_{mod.}) \ge r\ust -  \kappa_{\pi\ust} \epsilon.\label{ineq:1} 
	}
	
	Consider a modified version of the problem~\eqref{cmdp_approx_obj}-\eqref{cmdp_approx_con} in which the cost constraint is replaced by $U_B + \kappa_{\pi\ust} \epsilon$.
	It follows from the sensitivity analysis of CMDPs (Lemma~\ref{lemma:sensitivity_cmdp}) that $\tilde{r}(0)$ is greater than the optimal avg. reward of this modified CMDP minus $\kappa_{\pi\ust}\epsilon\frac{\hat{\eta}}{\eta}$, i.e,
	\ali{
		\tilde{r}(0) \ge \tilde{r}(U_B + \kappa_{\pi\ust} \epsilon) - \kappa_{\pi\ust}\epsilon\frac{\hat{\eta}}{\eta}  \label{ineq:2}
	}
	
	
	
	Since $\pi_{mod.}$ satisfies the constraints imposed while solving modified CMDP, $\bar{r}(\pi_{mod.})$ is less than the optimal value $\tilde{r}(U_B + \kappa_{\pi\ust} \epsilon)$ of the modified CMDP, i.e.,
	\ali{
		\bar{r}(\pi_{mod.}) \le \tilde{r}(U_B + \kappa_{\pi\ust} \epsilon). \label{ineq:3}
	}
	The proof then follows by combining~\eqref{ineq:1}-\eqref{ineq:3}. 
	$\blacksquare$
\end{proof}


==> subsecs/garbage.tex <==
\section{Solving~\eqref{eq:rbmle_2} Efficiently}\label{sec:solve_cmdp}
We will see how to solve the following problem efficiently:
\begin{align}
	&\te_k \in \arg\max_{\te \in \Theta} \bigg\{ \max_{\pi \in \Pi_{S}}\bigg\{ \alpha(\tau_k) \bar{r}(\theta,\pi) -\sum_{(x,u)} n_k(x,u)KL\left( \hat{p}_{k}(x,u),\te(x,u)  \right): \bar{c}(\te,\pi) \le c_{ub} \bigg\} \bigg\},\label{rbmle_prob}
\end{align}
and also obtain the corresponding optimal $\pi$.

\textbf{Embedding into an extended CMDP}: 
The problem~\eqref{rbmle_prob} can be viewed as an extended CMDP in which the optimizer\slash controller has to choose the following two quantities at each time $t$: \\
(i) controls $u(t)$, \\
(ii) MDP parameters $\te $.\\
We can merge these two controls, and let $u^{+}(t):= (\alpha(t),\te(t))\in \Delta(\cU) \times \Theta$ be the controls for this \textit{extended CMDP}. $\alpha(t)= \{\alpha_i(t)\}_{i=1}^{|U|}$ is the probability vector that decides the probabilities associated with each action.

The controlled transition probabilities for this extended MDP are given as follows (note that $\te$ is also part of control):
\ali{
	P^{+}(x,u^{+},y) = \sum_{i=1}^{|X|}   u_i ~\te(x,i,y),\label{def:extend_ptm}
}
where 
\nal{
	u^+ = (\alpha,\te).
}


Consider the following linear program in which the decision variables are given by $\{ \mu(x,u,\te): x \in \cX, u \in \widetilde{\Delta}_{\epsilon}(\cU),\te \in \widetilde{\Theta}_{\epsilon} \}$:
\begin{align}
	&\max \sum_{x \in \cX} \sum_{\alpha \in \widetilde{\Delta}_{\epsilon}(\cU)} \sum_{\te \in  \widetilde{\Theta}_{\epsilon}} \mu(x,\alpha,\te) \left\{\sum_{i=1}^{|U|} r(x,i) \right\},\label{overallobj_appx}
	&\intertext{subject to }\notag\\
	& \sum_{(\alpha,\te)} \mu(x,\alpha,\te) = \sum_{(y,\alpha,\te)} \mu(y,(\alpha,\te)  ) P^{+}(y, (\alpha,\te),x), \label{const1n_appx} \\
	& \mu(x,\alpha,\te) \geq 0, \\
	&\sum_{x \in \cX}\sum_{\alpha \in \widetilde{\Delta}_{\epsilon}(\cU)} \sum_{\te \in  \widetilde{\Theta}_{\epsilon}}\mu(x,\alpha,\te) = 1,  \label{const2n_appx} \\
	& \sum_{(x,\alpha,\te)} \mu(x,\alpha,\te) \left\{\sum_{i=1}^{|U|} \alpha_i r(x,i)\right\} \leq U_B . \label{constall_appx}
\end{align} %\eqref{overallobj_appx}-\eqref{constall_appx}
Let $\mu\ust$ be an optimal solution. $\pi\ust$ be the policy that randomizes amongst $u\in \cU$ when state is $x$, as follows: 
\begin{align}
	\frac{\sum\limits_{\alpha \in  \widetilde{\Delta}_{\epsilon}(\cU)}   \sum\limits_{\te \in  \widetilde{\Theta}_{\epsilon}}    \mu\ust(x,\alpha,\te)}{\sum_{(v,\te)} \mu\ust(x,v,\te)}.
\end{align}
(In case the denominator above is zero, choose any $\pi\ust_n(x_n,u_n,\te_n) \geq 0$ satisfying
$\sum_{v_n,\te_n} \pi\ust_n(x_n,v_n,\te_n) = 1$). 



\begin{definition}
	Let $\Pi^{+}_{S}$ denote the class of ``stationary randomized policies'' for the extended CMDP~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}. These policies fix $\te(t)\equiv \te,\forall t$ and also let $u(t)$ be solely a (possibly randomized) function of $x(t)$.
\end{definition}

\begin{lemma}\label{lemma:stat_opt}
	For the problem~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}, there exists an optimal controller within the class $\Pi^{+}_S$. 
\end{lemma}

\begin{comment}
We will approximate the infinite horizon CMDP~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2} by a finite time horizon problem that requires the agents to make decisions for $H$ steps. For this, we need the following assumption.

\begin{assumption}[Ergodicity]
The quantities 
\nal{
&\sup_{\pi^{+} \in \Pi^{+}_S} \Bigg| \bar{C}(\pi^{+})-\frac{1}{H}\bE_{\pi^{+}} \sum_{t=1}^{H}c(x(t),u(t))\Bigg|,\\
& \sup_{\pi^{+} \in \Pi^{+}_S} \Bigg|\bar{D}(\pi^{+})-\frac{1}{H}\bE_{\pi^{+}} \sum_{t=1}^{H}d(u(t))\Bigg|
}
are $o(H)$, i.e. their normalized (by $H$) versions vanish as $H\to\infty$. $\blacksquare$
\end{assumption}
%Let $\pi^{+,\star}$ be an optimal policy for the extended CMDP~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}. 

Under this assumption,~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2} can be approximated by the following problem involving $H$ horizon:
\ali{
\min_{\pi^+} \bE_{\pi^+}\left( \sum_{t=1}^{H} c(x(t),u^+(t))\right),\label{finite:obj}\\
\mbox{s.t.}\quad  \bE_{\pi^+}\left( \sum_{t=1}^{H} d(u^+(t)) \right)\le H U_B.  \label{finite:con}
}
Having reformulated~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}, we now derive some important structural results for it. 
\end{comment}
In~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}, the choice for $\te_n$ belongs to the set $\Theta_n$. Since~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2} has an uncountable action set, we will approximate it by a problem that involves finitely many decision variables. 




\textbf{Approximating Extended CMDP}: In what follows, we will assume that we have approximated the set $\Theta_n$ by a finite set $\tilde{\Theta}_n(\epsilon_1)$ that satisfies the following: for each $\te_n\in \Theta_n$ there exists at least one point $\tilde{\te}_n$ in the set $\tilde{\Theta}_n(\epsilon_1)$ that satisfies $\|\te_n-\tilde{\te}_n\|\le \epsilon_1$. 
We let $\tilde{\Pi}$ denote the set of policies that restrict to the set $\tilde{\Theta}_n(\epsilon_1)$ while choosing $\te_n$ (intead of choosing from a larger set $\Theta_n$). A policy $\tilde{\pi}\in \tilde{\Pi}$ chooses $u_n(t)\in \cU_n$ and $\te_n\in \tilde{\Theta}_n(\epsilon_1)$ for each agent $n$. The following assumption is in affect throughout this section.

\begin{assumption}\label{assum:strict}
	There exists a policy $\pi_{feas.} \in \tilde{\Pi}$ and a constant $\epsilon>0$ such that the average control cost under $\pi_{feas.}$ is strictly below $U_B - \epsilon$, where $U_B$ is as in the constraint~\eqref{def:constraints_learn_1}. We denote
	\ali{
		\eta := U_B - \epsilon - \bar{D}(\pi_{feas.}) \label{def:eta}
	}
\end{assumption}

The following CMDP that restricts to the class $\tilde{\Pi}$ is supposed to approximate the problem~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}:
\ali{
	\min_{ \tilde{\pi} \in \tilde{\Pi}} & \limsup_{T\to \infty} \frac{1}{T} \sum_{t=1}^{T} \bE_{\tilde{\pi}} \left( c(x(t),u(t)) \right)\label{cmdp_approx_obj}\\
	\mbox{ s.t. }& \limsup_{T\to \infty} \frac{1}{T} \sum_{t=1}^{T} \bE_{\tilde{\pi}} \left( d(x(t),u(t)) \right)  \le U_B.\label{cmdp_approx_con}
} %\eqref{cmdp_approx_obj}-\eqref{cmdp_approx_con}
\begin{theorem}\label{finite_LP}
	Consider the following linear program in which the decision variables are given by $\{ \mu_n(x_n,u_n,\te_n): x_n \in \cX_n, u_n \in\cU_n,\te_n \in \tilde{\Theta}_n(\epsilon_1), 1 \leq n \leq N \}$:
	\begin{align}
		&\min\sum_{n\in [N]} \sum_{x_n \in \cX_n} \sum_{u_n \in \cU_n} \sum_{\te_n \in \tilde{\Theta}_n(\epsilon_1)} \mu_n(x_n,u_n,\te_n) c_n(x_n,u_n) \label{overallobj_appx}
		&\intertext{subject to }\notag\\
		& \sum_{(u_n,\te_n)} \mu_n(x_n,u_n,\te_n) = \sum_{(y_n,v_n,\te_n)} \mu_n(y_n,(v_n,\te_n)  ) P^{+}_n(y_n, (v_n,\te_n)   ,x_n), \label{const1n_appx} \\
		& \mu_n(x_n,u_n,\te_n) \geq 0, \\
		&\sum_{x_n \in \cX_n}\sum_{u_n \in \cU_n} \sum_{\te_n \in \tilde{\Theta}_n(\epsilon_1) }\mu_n(x_n,u_n,\te_n) = 1, \forall n,  \label{const2n_appx} \\
		&\sum_{n\in [N]} \sum_{(x_n,u_n,\te_n)} \mu_n(x_n,u_n,\te_n) d_n(x_n,u_n) \leq U_B . \label{constall_appx}
	\end{align} %\eqref{overallobj_appx}-\eqref{constall_appx}
	Let $\mu\ust_n, ~n\in [N]$ be an optimal solution. Define the policy $\pi\ust_n$ as follows: 
	\begin{align}
		&\pi\ust_n(x_n,u_n) := \frac{\sum\limits_{\te_n \in \tilde{\Theta}_n}\mu\ust_n(x_n,u_n,\te_n)}{\sum_{(v_n,\te_n)} \mu\ust_n(x_n,v_n,\te_n)}.
	\end{align}
	(In case the denominator above is zero, choose any $\pi\ust_n(x_n,u_n,\te_n) \geq 0$ satisfying
	$\sum_{v_n,\te_n} \pi\ust_n(x_n,v_n,\te_n) = 1$). The policy $\otimes \pi^{\star}_n$ is optimal for the CMDP~\eqref{cmdp_approx_obj}-\eqref{cmdp_approx_con}.
\end{theorem}



The next result follows from Theorem~\ref{th:cho_meyer}.

\begin{lemma}
	Consider the finite LP~\eqref{overallobj_appx}-\eqref{constall_appx} that solves the CMDP~\eqref{cmdp_approx_obj}-\eqref{cmdp_approx_con}. The average reward satisfies 
	\nal{
		\tilde{r}(0) \ge     r\ust - \kappa_{\pi\ust} \epsilon - \kappa_{\pi\ust}\epsilon\frac{\hat{\eta}}{\eta} .
	}
\end{lemma}
\begin{proof}
	Let $\pi\ust$ solve the CMDP~\eqref{def:obj_learn}-\eqref{def:constraints_learn_2}. Under $\pi\ust$, in each state $x$, there is a probability measure over the space $\cU\times \Theta$ that corresponds to randomized choice of controls for the entire system, and the choice of the MDP parameter. We modify $\pi\ust$ as follows, so that now it chooses $\te_n$ from the finite set $\tilde{\Theta}_n$: when $\pi\ust$ suggests $\te_n$, then this is mapped to the nearest point $\tilde{\te}_n$ in the set $\tilde{\Theta}_n$. Clearly, we have that $\|\te_n-\tilde{\te}_n\|\le \epsilon$, and hence from Theorem~\ref{th:cho_meyer} that the average reward of this modified policy (say $\pi_{mod.}$) is greater than $r\ust -  \kappa_{\pi\ust} \epsilon $, and average cost is lesser than $U_B + \kappa_{\pi\ust} \epsilon$.
	\ali{
		\bar{r}(\pi_{mod.}) \ge r\ust -  \kappa_{\pi\ust} \epsilon.\label{ineq:1} 
	}
	
	Consider a modified version of the problem~\eqref{cmdp_approx_obj}-\eqref{cmdp_approx_con} in which the cost constraint is replaced by $U_B + \kappa_{\pi\ust} \epsilon$.
	It follows from the sensitivity analysis of CMDPs (Lemma~\ref{lemma:sensitivity_cmdp}) that $\tilde{r}(0)$ is greater than the optimal avg. reward of this modified CMDP minus $\kappa_{\pi\ust}\epsilon\frac{\hat{\eta}}{\eta}$, i.e,
	\ali{
		\tilde{r}(0) \ge \tilde{r}(U_B + \kappa_{\pi\ust} \epsilon) - \kappa_{\pi\ust}\epsilon\frac{\hat{\eta}}{\eta}  \label{ineq:2}
	}
	
	
	
	Since $\pi_{mod.}$ satisfies the constraints imposed while solving modified CMDP, $\bar{r}(\pi_{mod.})$ is less than the optimal value $\tilde{r}(U_B + \kappa_{\pi\ust} \epsilon)$ of the modified CMDP, i.e.,
	\ali{
		\bar{r}(\pi_{mod.}) \le \tilde{r}(U_B + \kappa_{\pi\ust} \epsilon). \label{ineq:3}
	}
	The proof then follows by combining~\eqref{ineq:1}-\eqref{ineq:3}. 
	$\blacksquare$
\end{proof}

